The Carina Nebula and Gum 31 molecular complex: II. The distribution of the atomic gas revealed in unprecedented detail

We report high spatial resolution observations of the HI 21cm line in the Carina Nebula and the Gum 31 region obtained with the Australia Telescope Compact Array. The observations covered $\sim$ 12 deg$^2$ centred on $l= 287.5\deg,b = -1\deg$, achieving an angular resolution of $\sim $ 35 arcseconds. The HI map revealed complex filamentary structures across a wide range of velocities. Several "bubbles" are clearly identified in the Carina Nebula Complex, produced by the impact of the massive star clusters located in this region. An HI absorption profile obtained towards the strong extragalactic radio source PMN J1032--5917 showed the distribution of the cold component of the atomic gas along the Galactic disk, with the Sagittarius-Carina and Perseus spiral arms clearly distinguishable. Preliminary calculations of the optical depth and spin temperatures of the cold atomic gas show that the HI line is opaque ($\tau \gtrsim$ 2) at several velocities in the Sagittarius-Carina spiral arm. The spin temperature is $\sim100$ K in the regions with the highest optical depth, although this value might be lower for the saturated components. The atomic mass budget of Gum 31 is $\sim35 \%$ of the total gas mass. HI self absorption features have molecular counterparts and good spatial correlation with the regions of cold dust as traced by the infrared maps. We suggest that in Gum 31 regions of cold temperature and high density are where the atomic to molecular gas phase transition is likely to be occurring.

==> biblio <==
@ARTICLE{2010MNRAS.406..952S,
   author = {{Smith}, N. and {Povich}, M.~S. and {Whitney}, B.~A. and {Churchwell}, E. and 
	{Babler}, B.~L. and {Meade}, M.~R. and {Bally}, J. and {Gehrz}, R.~D. and 
	{Robitaille}, T.~P. and {Stassun}, K.~G.},
    title = "{Spitzer Space Telescope observations of the Carina nebula: the steady march of feedback-driven star formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.2263},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: luminosity function, mass function, stars: pre-main-sequence, HII regions, ISM: evolution, ISM: individual objects: NGC 3372},
     year = 2010,
    month = aug,
   volume = 406,
    pages = {952-974},
      doi = {10.1111/j.1365-2966.2010.16792.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406..952S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.405.1153S,
   author = {{Smith}, N. and {Bally}, J. and {Walborn}, N.~R.},
    title = "{HST/ACS H{$\alpha$} imaging of the Carina Nebula: outflow activity traced by irradiated Herbig-Haro Jets}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1002.4898},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: pre-main-sequence, ISM: Herbig-Haro objects, ISM: individual: NGC 3372, ISM: individual: NGC 3324, ISM: jets and outflows},
     year = 2010,
    month = jun,
   volume = 405,
    pages = {1153-1186},
      doi = {10.1111/j.1365-2966.2010.16520.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.1153S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1998ApJ...493..180M,
   author = {{Massey}, P. and {Hunter}, D.~A.},
    title = "{Star Formation in R136: A Cluster of O3 Stars Revealed by Hubble Space Telescope Spectroscopy}",
  journal = {\apj},
 keywords = {STARS: EARLY-TYPE, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GALAXY: OPEN CLUSTERS AND ASSOCIATIONS: INDIVIDUAL ALPHANUMERIC: R136, Galaxy: Open Clusters and Associations: Individual: Alphanumeric: R136, Stars: Early-Type, Stars: Luminosity Function, Mass Function},
     year = 1998,
    month = jan,
   volume = 493,
    pages = {180-194},
      doi = {10.1086/305126},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...493..180M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...611L.105N,
   author = {{Najarro}, F. and {Figer}, D.~F. and {Hillier}, D.~J. and {Kudritzki}, R.~P.
	},
    title = "{Metallicity in the Galactic Center: The Arches Cluster}",
  journal = {\apjl},
   eprint = {astro-ph/0407188},
 keywords = {Galaxy: Abundances, Galaxy: Center, Infrared: Stars, Stars: Abundances, Stars: Wolf-Rayet},
     year = 2004,
    month = apr,
   volume = 611,
    pages = {L105-L108},
      doi = {10.1086/423955},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...611L.105N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INBOOK{2008hsf2.book..138S,
   author = {{Smith}, N. and {Brooks}, K.~J.},
    title = "{The Carina Nebula: A Laboratory for Feedback and Triggered Star Formation}",
booktitle = {Handbook of Star Forming Regions, Volume II},
     year = 2008,
    month = dec,
   editor = {{Reipurth}, B.},
    pages = {138},
   adsurl = {http://adsabs.harvard.edu/abs/2008hsf2.book..138S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..194...16T,
   author = {{Townsley}, L.~K. and {Broos}, P.~S. and {Chu}, Y.-H. and {Gruendl}, R.~A. and 
	{Oey}, M.~S. and {Pittard}, J.~M.},
    title = "{The Integrated Diffuse X-ray Emission of the Carina Nebula Compared to Other Massive Star-forming Regions}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1103.1606},
 primaryClass = "astro-ph.SR",
 keywords = {H II regions, X-rays: individual: Carina M17 NGC 3576 NGC 3603 30 Doradus},
     year = 2011,
    month = may,
   volume = 194,
      eid = {16},
    pages = {16},
      doi = {10.1088/0067-0049/194/1/16},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..194...16T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.327...46B,
   author = {{Brooks}, K.~J. and {Storey}, J.~W.~V. and {Whiteoak}, J.~B.
	},
    title = "{H110{$\alpha$} recombination-line emission and 4.8-GHz continuum emission in the Carina nebula}",
  journal = {\mnras},
   eprint = {astro-ph/0104344},
 keywords = {STARS: FORMATION, HII REGIONS, ISM: INDIVIDUAL: CARINA NEBULA, ISM: KINEMATICS AND DYNAMICS, RADIO LINES: ISM},
     year = 2001,
    month = oct,
   volume = 327,
    pages = {46-54},
      doi = {10.1046/j.1365-8711.2001.04590.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.327...46B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..194...15T,
   author = {{Townsley}, L.~K. and {Broos}, P.~S. and {Chu}, Y.-H. and {Gagn{\'e}}, M. and 
	{Garmire}, G.~P. and {Gruendl}, R.~A. and {Hamaguchi}, K. and 
	{Mac Low}, M.-M. and {Montmerle}, T. and {Naz{\'e}}, Y. and 
	{Oey}, M.~S. and {Park}, S. and {Petre}, R. and {Pittard}, J.~M.
	},
    title = "{The Chandra Carina Complex Project: Deciphering the Enigma of Carina's Diffuse X-ray Emission}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1103.0764},
 primaryClass = "astro-ph.SR",
 keywords = {H II regions, stars: massive, stars: winds, outflows, X-rays: individual: Carina, X-rays: ISM, X-rays: stars},
     year = 2011,
    month = may,
   volume = 194,
      eid = {15},
    pages = {15},
      doi = {10.1088/0067-0049/194/1/15},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..194...15T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..194....1T,
   author = {{Townsley}, L.~K. and {Broos}, P.~S. and {Corcoran}, M.~F. and 
	{Feigelson}, E.~D. and {Gagn{\'e}}, M. and {Montmerle}, T. and 
	{Oey}, M.~S. and {Smith}, N. and {Garmire}, G.~P. and {Getman}, K.~V. and 
	{Povich}, M.~S. and {Remage Evans}, N. and {Naz{\'e}}, Y. and 
	{Parkin}, E.~R. and {Preibisch}, T. and {Wang}, J. and {Wolk}, S.~J. and 
	{Chu}, Y.-H. and {Cohen}, D.~H. and {Gruendl}, R.~A. and {Hamaguchi}, K. and 
	{King}, R.~R. and {Mac Low}, M.-M. and {McCaughrean}, M.~J. and 
	{Moffat}, A.~F.~J. and {Oskinova}, L.~M. and {Pittard}, J.~M. and 
	{Stassun}, K.~G. and {ud-Doula}, A. and {Walborn}, N.~R. and 
	{Waldron}, W.~L. and {Churchwell}, E. and {Nichols}, J.~S. and 
	{Owocki}, S.~P. and {Schulz}, N.~S.},
    title = "{An Introduction to the Chandra Carina Complex Project}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1102.4779},
 primaryClass = "astro-ph.SR",
 keywords = {H II regions, stars: massive, stars: pre-main sequence, X-rays: individual: Carina, X-rays: ISM, X-rays: stars},
     year = 2011,
    month = may,
   volume = 194,
      eid = {1},
    pages = {1},
      doi = {10.1088/0067-0049/194/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..194....1T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008Natur.455..201S,
   author = {{Smith}, N.},
    title = "{A blast wave from the 1843 eruption of {$\eta$} Carinae}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {0809.1678},
     year = 2008,
    month = sep,
   volume = 455,
    pages = {201-203},
      doi = {10.1038/nature07269},
   adsurl = {http://adsabs.harvard.edu/abs/2008Natur.455..201S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2007MNRAS.379.1279S,
   author = {{Smith}, N. and {Brooks}, K.~J.},
    title = "{A census of the Carina Nebula - II. Energy budget and global properties of the nebulosity}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0705.3053},
 keywords = {stars: formation, HII regions, ISM: individual: NGC3372},
     year = 2007,
    month = aug,
   volume = 379,
    pages = {1279-1292},
      doi = {10.1111/j.1365-2966.2007.12021.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.379.1279S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2006MNRAS.367..763S,
   author = {{Smith}, N.},
    title = "{A census of the Carina Nebula - I. Cumulative energy input from massive stars}",
  journal = {\mnras},
   eprint = {astro-ph/0601060},
 keywords = {stars: early-type, stars: formation, stars: winds, outflows, ISM: bubbles, HII regions, ISM: individual: NGC 3372},
     year = 2006,
    month = apr,
   volume = 367,
    pages = {763-772},
      doi = {10.1111/j.1365-2966.2006.10007.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367..763S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...728..127D,
   author = {{Dawson}, J.~R. and {McClure-Griffiths}, N.~M. and {Kawamura}, A. and 
	{Mizuno}, N. and {Onishi}, T. and {Mizuno}, A. and {Fukui}, Y.
	},
    title = "{Supershells as Molecular Cloud Factories: Parsec Resolution Observations of H I and $^{12}$CO(J = 1-0) in GSH 287+04-17 and GSH 277+00+36}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.5363},
 primaryClass = "astro-ph.GA",
 keywords = {evolution, ISM: atoms, ISM: bubbles, ISM: clouds, ISM: molecules, radio lines: ISM},
     year = 2011,
    month = feb,
   volume = 728,
      eid = {127},
    pages = {127},
      doi = {10.1088/0004-637X/728/2/127},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...728..127D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...331..181G,
   author = {{Grabelsky}, D.~A. and {Cohen}, R.~S. and {Bronfman}, L. and 
	{Thaddeus}, P.},
    title = "{Molecular clouds in the Carina arm - The largest objects, associated regions of star formation, and the Carina arm in the Galaxy}",
  journal = {\apj},
 keywords = {Astronomical Catalogs, Galactic Structure, Interstellar Gas, Milky Way Galaxy, Molecular Clouds, Star Formation, H I Regions, Line Spectra, Sky Surveys (Astronomy)},
     year = 1988,
    month = aug,
   volume = 331,
    pages = {181-196},
      doi = {10.1086/166548},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...331..181G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...634..476Y,
   author = {{Yonekura}, Y. and {Asayama}, S. and {Kimura}, K. and {Ogawa}, H. and 
	{Kanai}, Y. and {Yamaguchi}, N. and {Barnes}, P.~J. and {Fukui}, Y.
	},
    title = "{High-Mass Cloud Cores in the {$\eta$} Carinae Giant Molecular Cloud}",
  journal = {\apj},
   eprint = {astro-ph/0508121},
 keywords = {ISM: Clouds, ISM: individual ({$\eta$} Carinae GMC), ISM: Molecules, Radio Lines: ISM, Stars: Formation},
     year = 2005,
    month = nov,
   volume = 634,
    pages = {476-494},
      doi = {10.1086/496869},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634..476Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...553..274Z,
   author = {{Zhang}, X. and {Lee}, Y. and {Bolatto}, A. and {Stark}, A.~A.
	},
    title = "{CO (J=4--{\gt}3) and [C I] Observations of the Carina Molecular Cloud Complex}",
  journal = {\apj},
   eprint = {astro-ph/0101272},
 keywords = {ISM: Clouds, ISM: Molecules, Submillimeter},
     year = 2001,
    month = may,
   volume = 553,
    pages = {274-287},
      doi = {10.1086/320628},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553..274Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.406.1350F,
   author = {{Froebrich}, D. and {Rowles}, J.},
    title = "{The structure of molecular clouds - II. Column density and mass distributions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.0117},
 keywords = {stars: formation, ISM: clouds, dust, extinction, ISM: structure},
     year = 2010,
    month = aug,
   volume = 406,
    pages = {1350-1357},
      doi = {10.1111/j.1365-2966.2010.16769.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.406.1350F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PASA...30...44B,
   author = {{Burton}, M.~G. and {Braiding}, C. and {Glueck}, C. and {Goldsmith}, P. and 
	{Hawkes}, J. and {Hollenbach}, D.~J. and {Kulesa}, C. and {Martin}, C.~L. and 
	{Pineda}, J.~L. and {Rowell}, G. and {Simon}, R. and {Stark}, A.~A. and 
	{Stutzki}, J. and {Tothill}, N.~J.~H. and {Urquhart}, J.~S. and 
	{Walker}, C. and {Walsh}, A.~J. and {Wolfire}, M.},
    title = "{The Mopra Southern Galactic Plane CO Survey}",
  journal = {\pasa},
archivePrefix = "arXiv",
   eprint = {1307.1027},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, ISM: clouds, ISM: molecules, radio lines: ISM, surveys},
     year = 2013,
    month = aug,
   volume = 30,
      eid = {e044},
    pages = {44},
      doi = {10.1017/pasa.2013.22},
   adsurl = {http://adsabs.harvard.edu/abs/2013PASA...30...44B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005ApJS..158..178M,
   author = {{McClure-Griffiths}, N.~M. and {Dickey}, J.~M. and {Gaensler}, B.~M. and 
	{Green}, A.~J. and {Haverkorn}, M. and {Strasser}, S.},
    title = "{The Southern Galactic Plane Survey: H I Observations and Analysis}",
  journal = {\apjs},
   eprint = {astro-ph/0503134},
 keywords = {Galaxy: Structure, ISM: Structure, Radio Lines: ISM, Surveys},
     year = 2005,
    month = jun,
   volume = 158,
    pages = {178-187},
      doi = {10.1086/430114},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJS..158..178M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PASP..122..314M,
   author = {{Molinari}, S. and {Swinyard}, B. and {Bally}, J. and {Barlow}, M. and 
	{Bernard}, J.-P. and {Martin}, P. and {Moore}, T. and {Noriega-Crespo}, A. and 
	{Plume}, R. and {Testi}, L. and {Zavagno}, A. and {Abergel}, A. and 
	{Ali}, B. and {Andr{\'e}}, P. and {Baluteau}, J.-P. and {Benedettini}, M. and 
	{Bern{\'e}}, O. and {Billot}, N.~P. and {Blommaert}, J. and 
	{Bontemps}, S. and {Boulanger}, F. and {Brand}, J. and {Brunt}, C. and 
	{Burton}, M. and {Campeggio}, L. and {Carey}, S. and {Caselli}, P. and 
	{Cesaroni}, R. and {Cernicharo}, J. and {Chakrabarti}, S. and 
	{Chrysostomou}, A. and {Codella}, C. and {Cohen}, M. and {Compiegne}, M. and 
	{Davis}, C.~J. and {de Bernardis}, P. and {de Gasperis}, G. and 
	{Di Francesco}, J. and {di Giorgio}, A.~M. and {Elia}, D. and 
	{Faustini}, F. and {Fischera}, J.~F. and {Fukui}, Y. and {Fuller}, G.~A. and 
	{Ganga}, K. and {Garcia-Lario}, P. and {Giard}, M. and {Giardino}, G. and 
	{Glenn}, J.~: and {Goldsmith}, P. and {Griffin}, M. and {Hoare}, M. and 
	{Huang}, M. and {Jiang}, B. and {Joblin}, C. and {Joncas}, G. and 
	{Juvela}, M. and {Kirk}, J. and {Lagache}, G. and {Li}, J.~Z. and 
	{Lim}, T.~L. and {Lord}, S.~D. and {Lucas}, P.~W. and {Maiolo}, B. and 
	{Marengo}, M. and {Marshall}, D. and {Masi}, S. and {Massi}, F. and 
	{Matsuura}, M. and {Meny}, C. and {Minier}, V. and {Miville-Desch{\^e}nes}, M.-A. and 
	{Montier}, L. and {Motte}, F. and {M{\"u}ller}, T.~G. and {Natoli}, P. and 
	{Neves}, J. and {Olmi}, L. and {Paladini}, R. and {Paradis}, D. and 
	{Pestalozzi}, M. and {Pezzuto}, S. and {Piacentini}, F. and 
	{Pomar{\`e}s}, M. and {Popescu}, C.~C. and {Reach}, W.~T. and 
	{Richer}, J. and {Ristorcelli}, I. and {Roy}, A. and {Royer}, P. and 
	{Russeil}, D. and {Saraceno}, P. and {Sauvage}, M. and {Schilke}, P. and 
	{Schneider-Bontemps}, N. and {Schuller}, F. and {Schultz}, B. and 
	{Shepherd}, D.~S. and {Sibthorpe}, B. and {Smith}, H.~A. and 
	{Smith}, M.~D. and {Spinoglio}, L. and {Stamatellos}, D. and 
	{Strafella}, F. and {Stringfellow}, G. and {Sturm}, E. and {Taylor}, R. and 
	{Thompson}, M.~A. and {Tuffs}, R.~J. and {Umana}, G. and {Valenziano}, L. and 
	{Vavrek}, R. and {Viti}, S. and {Waelkens}, C. and {Ward-Thompson}, D. and 
	{White}, G. and {Wyrowski}, F. and {Yorke}, H.~W. and {Zhang}, Q.
	},
    title = "{Hi-GAL: The Herschel Infrared Galactic Plane Survey}",
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1001.2106},
 primaryClass = "astro-ph.GA",
 keywords = {ISM},
     year = 2010,
    month = mar,
   volume = 122,
    pages = {314-325},
      doi = {10.1086/651314},
   adsurl = {http://adsabs.harvard.edu/abs/2010PASP..122..314M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983QJRAS..24..267H,
   author = {{Hildebrand}, R.~H.},
    title = "{The Determination of Cloud Masses and Dust Characteristics from Submillimetre Thermal Emission}",
  journal = {\qjras},
     year = 1983,
    month = sep,
   volume = 24,
    pages = {267},
   adsurl = {http://adsabs.harvard.edu/abs/1983QJRAS..24..267H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ApJ...244..483M,
   author = {{Mathis}, J.~S. and {Wallenhorst}, S.~G.},
    title = "{The size distribution of interstellar particles. III - Peculiar extinctions and normal infrared extinction}",
  journal = {\apj},
 keywords = {Cosmic Dust, Infrared Astronomy, Interstellar Extinction, Particle Size Distribution, Colorimetry, Graphite, Hydrogen, Silicates},
     year = 1981,
    month = mar,
   volume = 244,
    pages = {483-492},
      doi = {10.1086/158725},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...244..483M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...491..615G,
   author = {{Goldsmith}, P.~F. and {Bergin}, E.~A. and {Lis}, D.~C.},
    title = "{Carbon Monoxide and Dust Column Densities: The Dust-to-Gas Ratio and Structure of Three Giant Molecular Cloud Cores}",
  journal = {\apj},
 keywords = {ISM: Abundances, ISM: Clouds, ISM: Molecules, Radio Lines: ISM},
     year = 1997,
    month = dec,
   volume = 491,
    pages = {615-637},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...491..615G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...553..604D,
   author = {{Dupac}, X. and {Giard}, M. and {Bernard}, J.-P. and {Lamarre}, J.-M. and 
	{M{\'e}ny}, C. and {Pajot}, F. and {Ristorcelli}, I. and {Serra}, G. and 
	{Torre}, J.-P.},
    title = "{Submillimeter Mapping and Analysis of Cold Dust Condensations in the Orion M42 Star-forming Complex}",
  journal = {\apj},
   eprint = {astro-ph/0102407},
 keywords = {ISM: Dust, Extinction, Infrared: ISM: Continuum, ISM: Clouds, ISM: Individual: Name: Orion Nebula},
     year = 2001,
    month = jun,
   volume = 553,
    pages = {604-612},
      doi = {10.1086/320946},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553..604D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{2009ASPC..411..251M,
   author = {{Markwardt}, C.~B.},
    title = "{Non-linear Least-squares Fitting in IDL with MPFIT}",
booktitle = {Astronomical Data Analysis Software and Systems XVIII},
     year = 2009,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 411,
archivePrefix = "arXiv",
   eprint = {0902.2850},
 primaryClass = "astro-ph.IM",
   editor = {{Bohlender}, D.~A. and {Durand}, D. and {Dowler}, P.},
    month = sep,
    pages = {251},
   adsurl = {http://adsabs.harvard.edu/abs/2009ASPC..411..251M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2012A&A...541A.132P,
   author = {{Preibisch}, T. and {Roccatagliata}, V. and {Gaczkowski}, B. and 
	{Ratzka}, T.},
    title = "{Herschel far-infrared observations of the Carina Nebula complex. I. Introduction and global cloud structure}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1204.0627},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: clouds, ISM: structure, stars: formation},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201218851},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A.132P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...549A..67G,
   author = {{Gaczkowski}, B. and {Preibisch}, T. and {Ratzka}, T. and {Roccatagliata}, V. and 
	{Ohlendorf}, H. and {Zinnecker}, H.},
    title = "{Herschel far-infrared observations of the Carina Nebula complex. II. The embedded young stellar and protostellar population}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.2995},
 primaryClass = "astro-ph.GA",
 keywords = {stars: formation, circumstellar matter, stars: protostars, stars: luminosity function, mass function, ISM: individual objects: NGC 3372, stars: individual:{\amp}Carinae},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A67},
    pages = {A67},
      doi = {10.1051/0004-6361/201219836},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A..67G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...554A...6R,
   author = {{Roccatagliata}, V. and {Preibisch}, T. and {Ratzka}, T. and 
	{Gaczkowski}, B.},
    title = "{Herschel far-infrared observations of the Carina Nebula complex. III. Detailed cloud structure and feedback effects}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.5201},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: structure, stars: formation, ISM: general},
     year = 2013,
    month = jun,
   volume = 554,
      eid = {A6},
    pages = {A6},
      doi = {10.1051/0004-6361/201321081},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...554A...6R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1994A&A...291..943O,
   author = {{Ossenkopf}, V. and {Henning}, T.},
    title = "{Dust opacities for protostellar cores}",
  journal = {\aap},
 keywords = {Coagulation, Dust, Opacity, Protostars, Star Formation, Stellar Cores, Stellar Models, Absorptivity, Gas Density, Infrared Astronomy, Interstellar Extinction, Optical Properties, Radio Astronomy, Stellar Composition},
     year = 1994,
    month = nov,
   volume = 291,
    pages = {943-959},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...291..943O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003A&A...412..751B,
   author = {{Brooks}, K.~J. and {Cox}, P. and {Schneider}, N. and {Storey}, J.~W.~V. and 
	{Poglitsch}, A. and {Geis}, N. and {Bronfman}, L.},
    title = "{The Trumpler 14 photodissociation region in the Carina Nebula}",
  journal = {\aap},
 keywords = {stars: formation, ISM: lines and bands, ISM: clouds, ISM: individual objects: Carina nebula},
     year = 2003,
    month = dec,
   volume = 412,
    pages = {751-765},
      doi = {10.1051/0004-6361:20031406},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...412..751B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PASA...32...20B,
   author = {{Braiding}, C. and {Burton}, M.~G. and {Blackwell}, R. and {Gl{\"u}ck}, C. and 
	{Hawkes}, J. and {Kulesa}, C. and {Maxted}, N. and {Rebolledo}, D. and 
	{Rowell}, G. and {Stark}, A. and {Tothill}, N. and {Urquhart}, J.~S. and 
	{Voisin}, F. and {Walsh}, A.~J. and {de Wilt}, P. and {Wong}, G.~F.
	},
    title = "{The Mopra Southern Galactic Plane CO Survey - Data Release 1}",
  journal = {\pasa},
archivePrefix = "arXiv",
   eprint = {1504.04068},
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure, ISM: clouds, ISM: molecules, radio lines: ISM, surveys},
     year = 2015,
    month = may,
   volume = 32,
      eid = {e020},
    pages = {20},
      doi = {10.1017/pasa.2015.20},
   adsurl = {http://adsabs.harvard.edu/abs/2015PASA...32...20B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014AJ....148....5V,
   author = {{Vall{\'e}e}, J.~P.},
    title = "{The Spiral Arms of the Milky Way: The Relative Location of Each Different Arm Tracer within a Typical Spiral Arm Width}",
  journal = {\aj},
 keywords = {galaxies: individual: Milky Way, ISM: general},
     year = 2014,
    month = jul,
   volume = 148,
      eid = {5},
    pages = {5},
      doi = {10.1088/0004-6256/148/1/5},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....148....5V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...671..427M,
   author = {{McClure-Griffiths}, N.~M. and {Dickey}, J.~M.},
    title = "{Milky Way Kinematics. I. Measurements at the Subcentral Point of the Fourth Quadrant}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0708.0870},
 keywords = {Galaxy: Kinematics and Dynamics, ISM: Kinematics and Dynamics, Radio Lines: ISM},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {427-438},
      doi = {10.1086/522297},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671..427M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010A&A...518L..88B,
   author = {{Bernard}, J.-P. and {Paradis}, D. and {Marshall}, D.~J. and 
	{Montier}, L. and {Lagache}, G. and {Paladini}, R. and {Veneziani}, M. and 
	{Brunt}, C.~M. and {Mottram}, J.~C. and {Martin}, P. and {Ristorcelli}, I. and 
	{Noriega-Crespo}, A. and {Compi{\`e}gne}, M. and {Flagey}, N. and 
	{Anderson}, L.~D. and {Popescu}, C.~C. and {Tuffs}, R. and {Reach}, W. and 
	{White}, G. and {Benedettini}, M. and {Calzoletti}, L. and {Digiorgio}, A.~M. and 
	{Faustini}, F. and {Juvela}, M. and {Joblin}, C. and {Joncas}, G. and 
	{Mivilles-Deschenes}, M.-A. and {Olmi}, L. and {Traficante}, A. and 
	{Piacentini}, F. and {Zavagno}, A. and {Molinari}, S.},
    title = "{Dust temperature tracing the ISRF intensity in the Galaxy}",
  journal = {\aap},
 keywords = {ISM: general, dust, extinction, ISM: clouds, galaxies: ISM, infrared: ISM, submillimeter: ISM},
     year = 2010,
    month = jul,
   volume = 518,
      eid = {L88},
    pages = {L88},
      doi = {10.1051/0004-6361/201014540},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...518L..88B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ARA&A..51..207B,
   author = {{Bolatto}, A.~D. and {Wolfire}, M. and {Leroy}, A.~K.},
    title = "{The CO-to-H$_{2}$ Conversion Factor}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1301.3498},
 primaryClass = "astro-ph.GA",
     year = 2013,
    month = aug,
   volume = 51,
    pages = {207-268},
      doi = {10.1146/annurev-astro-082812-140944},
   adsurl = {http://adsabs.harvard.edu/abs/2013ARA%26A..51..207B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...546..980O,
   author = {{Ostriker}, E.~C. and {Stone}, J.~M. and {Gammie}, C.~F.},
    title = "{Density, Velocity, and Magnetic Field Structure in Turbulent Molecular Cloud Models}",
  journal = {\apj},
   eprint = {astro-ph/0008454},
 keywords = {ISM: Clouds, ISM: Molecules, Magnetohydrodynamics: MHD, Methods: Numerical, Stars: Formation},
     year = 2001,
    month = jan,
   volume = 546,
    pages = {980-1005},
      doi = {10.1086/318290},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...546..980O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...423..681V,
   author = {{Vazquez-Semadeni}, E.},
    title = "{Hierarchical Structure in Nearly Pressureless Flows as a Consequence of Self-similar Statistics}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, ISM: CLOUDS, ISM: STRUCTURE, TURBULENCE},
     year = 1994,
    month = mar,
   volume = 423,
    pages = {681},
      doi = {10.1086/173847},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...423..681V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2001ApJ...557..727V,
   author = {{V{\'a}zquez-Semadeni}, E. and {Garc{\'{\i}}a}, N.},
    title = "{The Probability Distribution Function of Column Density in Molecular Clouds}",
  journal = {\apj},
   eprint = {astro-ph/0103199},
 keywords = {ISM: Clouds, ISM: Molecules},
     year = 2001,
    month = aug,
   volume = 557,
    pages = {727-735},
      doi = {10.1086/321688},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...557..727V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...634.1126M,
   author = {{Milam}, S.~N. and {Savage}, C. and {Brewster}, M.~A. and {Ziurys}, L.~M. and 
	{Wyckoff}, S.},
    title = "{The $^{12}$C/$^{13}$C Isotope Gradient Derived from Millimeter Transitions of CN: The Case for Galactic Chemical Evolution}",
  journal = {\apj},
 keywords = {Astrochemistry, Galaxy: Evolution, ISM: Abundances, ISM: Clouds, Radio Lines: ISM, Stars: AGB and Post-AGB},
     year = 2005,
    month = dec,
   volume = 634,
    pages = {1126-1132},
      doi = {10.1086/497123},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1126M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982ApJ...262..590F,
   author = {{Frerking}, M.~A. and {Langer}, W.~D. and {Wilson}, R.~W.},
    title = "{The relationship between carbon monoxide abundance and visual extinction in interstellar clouds}",
  journal = {\apj},
 keywords = {Abundance, Carbon Monoxide, Interstellar Extinction, Interstellar Matter, Molecular Clouds, Astronomical Catalogs, Gas Density, Isotopes, Mass},
     year = 1982,
    month = nov,
   volume = 262,
    pages = {590-605},
      doi = {10.1086/160451},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...262..590F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...721..686P,
   author = {{Pineda}, J.~L. and {Goldsmith}, P.~F. and {Chapman}, N. and 
	{Snell}, R.~L. and {Li}, D. and {Cambr{\'e}sy}, L. and {Brunt}, C.
	},
    title = "{The Relation Between Gas and Dust in the Taurus Molecular Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1007.5060},
 primaryClass = "astro-ph.GA",
 keywords = {dust, extinction, ISM: molecules, ISM: structure},
     year = 2010,
    month = sep,
   volume = 721,
    pages = {686-708},
      doi = {10.1088/0004-637X/721/1/686},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...721..686P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2004tra..book.....R,
   author = {{Rohlfs}, K. and {Wilson}, T.~L.},
    title = "{Tools of radio astronomy}",
 keywords = {RADIO ASTRONOMY},
booktitle = {Tools of radio astronomy, 4th rev.~and enl.~ed., by K.~Rohlfs and T.L.~Wilson.~ Berlin: Springer, 2004},
     year = 2004,
   adsurl = {http://adsabs.harvard.edu/abs/2004tra..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...508L..35K,
   author = {{Kainulainen}, J. and {Beuther}, H. and {Henning}, T. and {Plume}, R.
	},
    title = "{Probing the evolution of molecular cloud structure. From quiescence to birth}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0911.5648},
 keywords = {ISM: clouds, ISM: structure, stars: formation, dust, extinction, evolution},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {L35-L38},
      doi = {10.1051/0004-6361/200913605},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508L..35K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004MNRAS.348..638B,
   author = {{Burton}, M.~G. and {Lazendic}, J.~S. and {Yusef-Zadeh}, F. and 
	{Wardle}, M.},
    title = "{The Eye of the Tornado - an isolated, high-mass young stellar object near the Galactic Centre}",
  journal = {\mnras},
   eprint = {astro-ph/0308262},
 keywords = {stars: formation, HII regions, ISM: individual: Tornado Nebula, ISM: individual: G357.7-0.1, ISM: molecules, supernova remnants},
     year = 2004,
    month = feb,
   volume = 348,
    pages = {638-646},
      doi = {10.1111/j.1365-2966.2004.07381.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348..638B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...530A..34P,
   author = {{Preibisch}, T. and {Ratzka}, T. and {Kuderna}, B. and {Ohlendorf}, H. and 
	{King}, R.~R. and {Hodgkin}, S. and {Irwin}, M. and {Lewis}, J.~R. and 
	{McCaughrean}, M.~J. and {Zinnecker}, H.},
    title = "{Deep wide-field near-infrared survey of the Carina Nebula}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.3477},
 keywords = {stars: formation, stars: luminosity function, mass function, circumstellar matter, stars: pre-main sequence, ISM: individual objects:NGC 3372, ISM: jets and outflows},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A34},
    pages = {A34},
      doi = {10.1051/0004-6361/201116781},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A..34P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...552A..14O,
   author = {{Ohlendorf}, H. and {Preibisch}, T. and {Gaczkowski}, B. and 
	{Ratzka}, T. and {Ngoumou}, J. and {Roccatagliata}, V. and {Grellmann}, R.
	},
    title = "{Discovering young stars in the Gum 31 region with infrared observations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.0007},
 keywords = {stars: formation, stars: protostars, ISM: jets and outflows, Herbig-Haro objects, ISM: clouds, ISM: bubbles},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201220218},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A..14O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986ApJ...307..609H,
   author = {{Herbig}, G.~H. and {Terndrup}, D.~M.},
    title = "{The Trapezium cluster of the Orion nebula}",
  journal = {\apj},
 keywords = {Color-Magnitude Diagram, Interstellar Gas, Orion Nebula, Star Clusters, Astronomical Catalogs, Astronomical Photometry, Molecular Clouds, Pre-Main Sequence Stars, Stellar Evolution},
     year = 1986,
    month = aug,
   volume = 307,
    pages = {609-618},
      doi = {10.1086/164447},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...307..609H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...430..481H,
   author = {{Homeier}, N.~L. and {Alves}, J.},
    title = "{Massive star formation in the W49 giant molecular cloud: Implications for the formation of massive star clusters}",
  journal = {\aap},
   eprint = {astro-ph/0409410},
 keywords = {ISM: H II regions, ISM: bubbles, Galaxy: open clusters and associations: individual: W49A, stars: formation, Galaxy: disk, infrared: ISM},
     year = 2005,
    month = feb,
   volume = 430,
    pages = {481-489},
      doi = {10.1051/0004-6361:20040447},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...430..481H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983A&A...124..273M,
   author = {{Moffat}, A.~F.~J.},
    title = "{The bright stellar content of the giant galactic H II region NGC 3603}",
  journal = {\aap},
 keywords = {B Stars, H Ii Regions, Interstellar Matter, O Stars, Wolf-Rayet Stars, Hertzsprung-Russell Diagram, Interstellar Extinction, Star Clusters, Stellar Spectrophotometry},
     year = 1983,
    month = aug,
   volume = 124,
    pages = {273-278},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...124..273M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.331...85R,
   author = {{Rathborne}, J.~M. and {Burton}, M.~G. and {Brooks}, K.~J. and 
	{Cohen}, M. and {Ashley}, M.~C.~B. and {Storey}, J.~W.~V.},
    title = "{Photodissociation regions and star formation in the Carina nebula}",
  journal = {\mnras},
   eprint = {astro-ph/0111318},
 keywords = {stars: formation, HII regions, ISM: individual: Carina nebula, ISM: lines and bands, ISM: molecules, ISM: structure, stars: formation, HII regions, ISM: individual: Carina nebula, ISM: lines and bands, ISM: molecules, ISM: structure},
     year = 2002,
    month = mar,
   volume = 331,
    pages = {85-97},
      doi = {10.1046/j.1365-8711.2002.05149.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.331...85R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...418..563R,
   author = {{Rathborne}, J.~M. and {Brooks}, K.~J. and {Burton}, M.~G. and 
	{Cohen}, M. and {Bontemps}, S.},
    title = "{The giant pillars of the Carina Nebula}",
  journal = {\aap},
   eprint = {astro-ph/0310605},
 keywords = {ISM: structure, ISM: lines and bands, ISM: molecules, H II, regions, dust, extinction, stars: formation},
     year = 2004,
    month = may,
   volume = 418,
    pages = {563-576},
      doi = {10.1051/0004-6361:20031631},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...418..563R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PHDTHESIS{2000PhDT.........2B,
   author = {{Brooks}, K.~J.},
    title = "{An investigation of the Carina Nebula}",
 keywords = {CARINA, TRUMPLER 14, TRUMPLER 16, ETA CARINAE, KEYHOLE},
   school = {European Southern Observatory, Casilla 19001, Santiago 19, Chile},
     year = 2000,
    month = October,
   adsurl = {http://adsabs.harvard.edu/abs/2000PhDT.........2B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...217..425M,
   author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
    title = "{The size distribution of interstellar grains}",
  journal = {\apj},
 keywords = {Cosmic Dust, Interstellar Extinction, Interstellar Matter, Particle Size Distribution, Enstatite, Graphite, Magnetite, Olivine, Polarization Characteristics, Ultraviolet Astronomy},
     year = 1977,
    month = oct,
   volume = 217,
    pages = {425-433},
      doi = {10.1086/155591},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...808...99R,
   author = {{Rebolledo}, D. and {Wong}, T. and {Xue}, R. and {Leroy}, A. and 
	{Koda}, J. and {Donovan Meyer}, J.},
    title = "{Scaling Relations of the Properties for CO Resolved Structures in Nearby Spiral Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1506.05599},
 keywords = {galaxies: individual: NGC 6946, NGC 628, M101, galaxies: ISM, ISM: molecules, stars: formation},
     year = 2015,
    month = jul,
   volume = 808,
      eid = {99},
    pages = {99},
      doi = {10.1088/0004-637X/808/1/99},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...808...99R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001A&A...371..107C,
   author = {{Carraro}, G. and {Patat}, F. and {Baumgardt}, H.},
    title = "{Star clusterings in the Carina complex: vec $\{$UBVRI$\}$ photometry of NGC 3324 and Loden 165}",
  journal = {\aap},
   eprint = {astro-ph/0102387},
 keywords = {PHOTOMETRY: OPTICAL, OPEN CLUSTERS AND ASSOCIATIONS: NGC 3324: INDIVIDUAL, OPEN CLUSTERS AND ASSOCIATIONS: LODEN 165: INDIVIDUAL},
     year = 2001,
    month = may,
   volume = 371,
    pages = {107-114},
      doi = {10.1051/0004-6361:20010307},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...371..107C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...438.1163K,
   author = {{Kharchenko}, N.~V. and {Piskunov}, A.~E. and {R{\"o}ser}, S. and 
	{Schilbach}, E. and {Scholz}, R.-D.},
    title = "{Astrophysical parameters of Galactic open clusters}",
  journal = {\aap},
   eprint = {astro-ph/0501674},
 keywords = {techniques: photometric, catalogs, astrometry, stars: kinematics, open clusters and associations: general, Galaxy: stellar content},
     year = 2005,
    month = aug,
   volume = 438,
    pages = {1163-1173},
      doi = {10.1051/0004-6361:20042523},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...438.1163K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.402...73B,
   author = {{Barnes}, P.~J. and {Yonekura}, Y. and {Ryder}, S.~D. and {Hopkins}, A.~M. and 
	{Miyamoto}, Y. and {Furukawa}, N. and {Fukui}, Y.},
    title = "{Discovery of large-scale gravitational infall in a massive protostellar cluster}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0812.1789},
 keywords = {astrochemistry, stars: formation, ISM: kinematics and dynamics, ISM: molecules, infrared: ISM, radio lines: ISM},
     year = 2010,
    month = feb,
   volume = 402,
    pages = {73-86},
      doi = {10.1111/j.1365-2966.2009.15890.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.402...73B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...692...91G,
   author = {{Goodman}, A.~A. and {Pineda}, J.~E. and {Schnee}, S.~L.},
    title = "{The ''True'' Column Density Distribution in Star-Forming Molecular Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0806.3441},
 keywords = {dust, extinction, ISM: abundances, ISM: individual: Perseus molecular complex, ISM: molecules},
     year = 2009,
    month = feb,
   volume = 692,
    pages = {91-103},
      doi = {10.1088/0004-637X/692/1/91},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...692...91G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.288..145P,
   author = {{Padoan}, P. and {Nordlund}, A. and {Jones}, B.~J.~T.},
    title = "{The universality of the stellar initial mass function}",
  journal = {\mnras},
   eprint = {astro-ph/9703110},
 keywords = {STARS: FORMATION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, ISM: KINEMATICS AND DYNAMICS},
     year = 1997,
    month = jun,
   volume = 288,
    pages = {145-152},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.288..145P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005Sci...307.1292G,
   author = {{Grenier}, I.~A. and {Casandjian}, J.-M. and {Terrier}, R.},
    title = "{Unveiling Extensive Clouds of Dark Gas in the Solar Neighborhood}",
  journal = {Science},
     year = 2005,
    month = feb,
   volume = 307,
    pages = {1292-1295},
      doi = {10.1126/science.1106924},
   adsurl = {http://adsabs.harvard.edu/abs/2005Sci...307.1292G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016MNRAS.456.2406R,
   author = {{Rebolledo}, D. and {Burton}, M. and {Green}, A. and {Braiding}, C. and 
	{Molinari}, S. and {Wong}, G. and {Blackwell}, R. and {Elia}, D. and 
	{Schisano}, E.},
    title = "{The Carina Nebula and Gum 31 molecular complex - I. Molecular gas distribution, column densities, and dust temperatures}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.07513},
 keywords = {stars: formation, ISM: molecules, galaxies: ISM, ISM: individual: Carina Nebula, Gum 31, infrared: ISM},
     year = 2016,
    month = mar,
   volume = 456,
    pages = {2406-2424},
      doi = {10.1093/mnras/stv2776},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.2406R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008AJ....136.2563W,
   author = {{Walter}, F. and {Brinks}, E. and {de Blok}, W.~J.~G. and {Bigiel}, F. and 
	{Kennicutt}, Jr., R.~C. and {Thornley}, M.~D. and {Leroy}, A.
	},
    title = "{THINGS: The H I Nearby Galaxy Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0810.2125},
 keywords = {galaxies: ISM, galaxies: structure, ISM: atoms, ISM: general, radio lines: galaxies, surveys},
     year = 2008,
    month = dec,
   volume = 136,
      eid = {2563-2647},
    pages = {2563-2647},
      doi = {10.1088/0004-6256/136/6/2563},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.2563W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008AJ....136.2648D,
   author = {{de Blok}, W.~J.~G. and {Walter}, F. and {Brinks}, E. and {Trachternach}, C. and 
	{Oh}, S.-H. and {Kennicutt}, Jr., R.~C.},
    title = "{High-Resolution Rotation Curves and Galaxy Mass Models from THINGS}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0810.2100},
 keywords = {dark matter, galaxies: dwarf, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: structure},
     year = 2008,
    month = dec,
   volume = 136,
      eid = {2648-2719},
    pages = {2648-2719},
      doi = {10.1088/0004-6256/136/6/2648},
   adsurl = {http://adsabs.harvard.edu/abs/2008AJ....136.2648D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...540..851G,
   author = {{Gibson}, S.~J. and {Taylor}, A.~R. and {Higgs}, L.~A. and {Dewdney}, P.~E.
	},
    title = "{A New View of Cold H I Clouds in the Milky Way}",
  journal = {\apj},
 keywords = {ISM: Clouds, ISM: Globules, ISM: Structure, Methods: Analytical, radiative transfer, Radio Lines: ISM},
     year = 2000,
    month = sep,
   volume = 540,
    pages = {851-862},
      doi = {10.1086/309364},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...540..851G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...536..756D,
   author = {{Dickey}, J.~M. and {Mebold}, U. and {Stanimirovic}, S. and 
	{Staveley-Smith}, L.},
    title = "{Cold Atomic Gas in the Small Magellanic Cloud}",
  journal = {\apj},
 keywords = {Galaxies: ISM, ISM: Clouds, Galaxies: Magellanic Clouds, Radio Lines: Galaxies},
     year = 2000,
    month = jun,
   volume = 536,
    pages = {756-772},
      doi = {10.1086/308953},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...536..756D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1996ASPC..106....1W,
   author = {{Walterbos}, R.~A.~M. and {Braun}, R.},
    title = "{The Cool and Warm Phases of the Interstellar Medium in Spiral Galaxies}",
booktitle = {The Minnesota Lectures on Extragalactic Neutral Hydrogen},
     year = 1996,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 106,
   editor = {{Skillman}, E.~D.},
    pages = {1},
   adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..106....1W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...804...89M,
   author = {{Murray}, C.~E. and {Stanimirovi{\'c}}, S. and {Goss}, W.~M. and 
	{Dickey}, J.~M. and {Heiles}, C. and {Lindner}, R.~R. and {Babler}, B. and 
	{Pingel}, N.~M. and {Lawrence}, A. and {Jencson}, J. and {Hennebelle}, P.
	},
    title = "{The 21-SPONGE HI Absorption Survey I: Techniques and Initial Results}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1503.01108},
 keywords = {ISM: clouds, ISM: structure, radio lines: ISM},
     year = 2015,
    month = may,
   volume = 804,
      eid = {89},
    pages = {89},
      doi = {10.1088/0004-637X/804/2/89},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...804...89M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...781L..41M,
   author = {{Murray}, C.~E. and {Lindner}, R.~R. and {Stanimirovi{\'c}}, S. and 
	{Goss}, W.~M. and {Heiles}, C. and {Dickey}, J. and {Pingel}, N.~M. and 
	{Lawrence}, A. and {Jencson}, J. and {Babler}, B.~L. and {Hennebelle}, P.
	},
    title = "{Excitation Temperature of the Warm Neutral Medium as a New Probe of the Ly{$\alpha$} Radiation Field}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1401.1215},
 keywords = {ISM: clouds, ISM: structure },
     year = 2014,
    month = feb,
   volume = 781,
      eid = {L41},
    pages = {L41},
      doi = {10.1088/2041-8205/781/2/L41},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781L..41M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996A&AS..120..375S,
   author = {{Sault}, R.~J. and {Staveley-Smith}, L. and {Brouw}, W.~N.},
    title = "{An approach to interferometric mosaicing.}",
  journal = {\aaps},
 keywords = {TECHNIQUES: INTERFEROMETRIC, METHODS: DATA ANALYSIS, MAGELLANIC CLOUDS, RADIO LINES: GALAXIES},
     year = 1996,
    month = dec,
   volume = 120,
    pages = {375-384},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..120..375S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1995ASPC...77..433S,
   author = {{Sault}, R.~J. and {Teuben}, P.~J. and {Wright}, M.~C.~H.},
    title = "{A Retrospective View of MIRIAD}",
booktitle = {Astronomical Data Analysis Software and Systems IV},
     year = 1995,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 77,
   eprint = {astro-ph/0612759},
   editor = {{Shaw}, R.~A. and {Payne}, H.~E. and {Hayes}, J.~J.~E.},
    pages = {433},
   adsurl = {http://adsabs.harvard.edu/abs/1995ASPC...77..433S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...532L.145S,
   author = {{Smith}, N. and {Egan}, M.~P. and {Carey}, S. and {Price}, S.~D. and 
	{Morse}, J.~A. and {Price}, P.~A.},
    title = "{Large-Scale Structure of the Carina Nebula}",
  journal = {\apjl},
 keywords = {ISM: H II REGIONS, ISM: INDIVIDUAL: NAME: CARINA NEBULA, STARS: FORMATION},
     year = 2000,
    month = apr,
   volume = 532,
    pages = {L145-L148},
      doi = {10.1086/312578},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...532L.145S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJS..145..329H,
   author = {{Heiles}, C. and {Troland}, T.~H.},
    title = "{The Millennium Arecibo 21 Centimeter Absorption-Line Survey. I. Techniques and Gaussian Fits}",
  journal = {\apjs},
   eprint = {astro-ph/0207104},
 keywords = {ISM: Atoms, ISM: Structure, Radio Lines: ISM},
     year = 2003,
    month = apr,
   volume = 145,
    pages = {329-354},
      doi = {10.1086/367785},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJS..145..329H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...586.1067H,
   author = {{Heiles}, C. and {Troland}, T.~H.},
    title = "{The Millennium Arecibo 21 Centimeter Absorption-Line Survey. II. Properties of the Warm and Cold Neutral Media}",
  journal = {\apj},
   eprint = {astro-ph/0207105},
 keywords = {ISM: Atoms, ISM: Structure, Radio Lines: ISM},
     year = 2003,
    month = apr,
   volume = 586,
    pages = {1067-1093},
      doi = {10.1086/367828},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586.1067H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...603..560S,
   author = {{Strasser}, S. and {Taylor}, A.~R.},
    title = "{1420 MHz Continuum Absorption toward Extragalactic Sources in the Galactic Plane}",
  journal = {\apj},
   eprint = {astro-ph/0401248},
 keywords = {Galaxy: Disk, Galaxy: Fundamental Parameters, ISM: Atoms, Radio Lines: ISM},
     year = 2004,
    month = mar,
   volume = 603,
    pages = {560-568},
      doi = {10.1086/381674},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...603..560S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007AJ....134.2252S,
   author = {{Strasser}, S.~T. and {Dickey}, J.~M. and {Taylor}, A.~R. and 
	{Boothroyd}, A.~I. and {Gaensler}, B.~M. and {Green}, A.~J. and 
	{Kavars}, D.~W. and {Lockman}, F.~J. and {Martin}, P.~G. and 
	{McClure-Griffiths}, N.~M. and {Rothwell}, T.~A. and {Stil}, J.~M.
	},
    title = "{Tracking the Outer Spiral Arms of the Galaxy in H I Absorption}",
  journal = {\aj},
 keywords = {Galaxy: disk, ISM: atoms, ISM: clouds, radio lines: ISM},
     year = 2007,
    month = dec,
   volume = 134,
    pages = {2252-2271},
      doi = {10.1086/522794},
   adsurl = {http://adsabs.harvard.edu/abs/2007AJ....134.2252S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2015A&A...580A.112B,
   author = {{Bihr}, S. and {Beuther}, H. and {Ott}, J. and {Johnston}, K.~G. and 
	{Brunthaler}, A. and {Anderson}, L.~D. and {Bigiel}, F. and 
	{Carlhoff}, P. and {Churchwell}, E. and {Glover}, S.~C.~O. and 
	{Goldsmith}, P.~F. and {Heitsch}, F. and {Henning}, T. and {Heyer}, M.~H. and 
	{Hill}, T. and {Hughes}, A. and {Klessen}, R.~S. and {Linz}, H. and 
	{Longmore}, S.~N. and {McClure-Griffiths}, N.~M. and {Menten}, K.~M. and 
	{Motte}, F. and {Nguyen-Luong}, Q. and {Plume}, R. and {Ragan}, S.~E. and 
	{Roy}, N. and {Schilke}, P. and {Schneider}, N. and {Smith}, R.~J. and 
	{Stil}, J.~M. and {Urquhart}, J.~S. and {Walsh}, A.~J. and {Walter}, F.
	},
    title = "{THOR: The H i, OH, Recombination line survey of the Milky Way. The pilot study: H i observations of the giant molecular cloud W43}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.05176},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: structure, ISM: atoms, stars: formation, radio lines: ISM, surveys},
     year = 2015,
    month = aug,
   volume = 580,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201425370},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...580A.112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...663..258B,
   author = {{Brown}, J.~C. and {Haverkorn}, M. and {Gaensler}, B.~M. and 
	{Taylor}, A.~R. and {Bizunok}, N.~S. and {McClure-Griffiths}, N.~M. and 
	{Dickey}, J.~M. and {Green}, A.~J.},
    title = "{Rotation Measures of Extragalactic Sources behind the Southern Galactic Plane: New Insights into the Large-Scale Magnetic Field of the Inner Milky Way}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.0458},
 keywords = {Galaxy: Structure, ISM: Magnetic Fields, Polarization},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {258-266},
      doi = {10.1086/518499},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663..258B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...809...56L,
   author = {{Lee}, M.-Y. and {Stanimirovi{\'c}}, S. and {Murray}, C.~E. and 
	{Heiles}, C. and {Miller}, J.},
    title = "{Cold and Warm Atomic Gas around the Perseus Molecular Cloud. II. The Impact of High Optical Depth on the HI Column Density Distribution and Its Implication for the HI-to-H$_{2}$ Transition}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1504.07405},
 keywords = {ISM: individual objects: Perseus, ISM: molecules, radio lines: ISM},
     year = 2015,
    month = aug,
   volume = 809,
      eid = {56},
    pages = {56},
      doi = {10.1088/0004-637X/809/1/56},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...809...56L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...693..216K,
   author = {{Krumholz}, M.~R. and {McKee}, C.~F. and {Tumlinson}, J.},
    title = "{The Atomic-to-Molecular Transition in Galaxies. II: H I and H$_{2}$ Column Densities}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0811.0004},
 keywords = {galaxies: ISM, ISM: clouds, ISM: molecules, ISM: structure, molecular processes},
     year = 2009,
    month = mar,
   volume = 693,
    pages = {216-235},
      doi = {10.1088/0004-637X/693/1/216},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...693..216K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...709..308M,
   author = {{McKee}, C.~F. and {Krumholz}, M.~R.},
    title = "{The Atomic-to-Molecular Transition in Galaxies. III. A New Method for Determining the Molecular Content of Primordial and Dusty Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.0330},
 keywords = {ISM: clouds, ISM: molecules, molecular processes, radiative transfer, stars: formation},
     year = 2010,
    month = jan,
   volume = 709,
    pages = {308-320},
      doi = {10.1088/0004-637X/709/1/308},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...709..308M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...748...75L,
   author = {{Lee}, M.-Y. and {Stanimirovi{\'c}}, S. and {Douglas}, K.~A. and 
	{Knee}, L.~B.~G. and {Di Francesco}, J. and {Gibson}, S.~J. and 
	{Begum}, A. and {Grcevich}, J. and {Heiles}, C. and {Korpela}, E.~J. and 
	{Leroy}, A.~K. and {Peek}, J.~E.~G. and {Pingel}, N.~M. and 
	{Putman}, M.~E. and {Saul}, D.},
    title = "{A High-resolution Study of the H I-H$_{2}$ Transition across the Perseus Molecular Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1110.2745},
 keywords = {dust, extinction, infrared: ISM, ISM: individual objects: Perseus, ISM: molecules, radio lines: ISM},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {75},
    pages = {75},
      doi = {10.1088/0004-637X/748/2/75},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...75L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...620L..95G,
   author = {{Gaensler}, B.~M. and {McClure-Griffiths}, N.~M. and {Oey}, M.~S. and 
	{Haverkorn}, M. and {Dickey}, J.~M. and {Green}, A.~J.},
    title = "{A Stellar Wind Bubble Coincident with the Anomalous X-Ray Pulsar 1E 1048.1-5937: Are Magnetars Formed from Massive Progenitors?}",
  journal = {\apjl},
   eprint = {astro-ph/0501563},
 keywords = {ISM: Bubbles, ISM: Individual: Alphanumeric: GSH 288.3-0.5-28, Stars: Pulsars: Individual: Alphanumeric: 1E 1048.1-5937, Radio Lines: ISM, Stars: Neutron, Stars: Winds, Outflows},
     year = 2005,
    month = feb,
   volume = 620,
    pages = {L95-L98},
      doi = {10.1086/428725},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...620L..95G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1968AuJPh..21..881G,
   author = {{Gardner}, F.~F. and {Morimoto}, M.},
    title = "{5 GHz continuum radiation from southern hemisphere galactic HII regions}",
  journal = {Australian Journal of Physics},
     year = 1968,
    month = dec,
   volume = 21,
    pages = {881},
      doi = {10.1071/PH680881},
   adsurl = {http://adsabs.harvard.edu/abs/1968AuJPh..21..881G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJS..151..103M,
   author = {{Ma{\'{\i}}z-Apell{\'a}niz}, J. and {Walborn}, N.~R. and {Galu{\'e}}, H.~{\'A}. and 
	{Wei}, L.~H.},
    title = "{A Galactic O Star Catalog}",
  journal = {\apjs},
   eprint = {astro-ph/0311196},
 keywords = {Stars: Binaries: General, Catalogs, Galaxy: Open Clusters and Associations: General, Stars: Distances, Stars: Early-Type, Stars: Fundamental Parameters},
     year = 2004,
    month = mar,
   volume = 151,
    pages = {103-148},
      doi = {10.1086/381380},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..151..103M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.416..832W,
   author = {{Wilson}, W.~E. and {Ferris}, R.~H. and {Axtens}, P. and {Brown}, A. and 
	{Davis}, E. and {Hampson}, G. and {Leach}, M. and {Roberts}, P. and 
	{Saunders}, S. and {Koribalski}, B.~S. and {Caswell}, J.~L. and 
	{Lenc}, E. and {Stevens}, J. and {Voronkov}, M.~A. and {Wieringa}, M.~H. and 
	{Brooks}, K. and {Edwards}, P.~G. and {Ekers}, R.~D. and {Emonts}, B. and 
	{Hindson}, L. and {Johnston}, S. and {Maddison}, S.~T. and {Mahony}, E.~K. and 
	{Malu}, S.~S. and {Massardi}, M. and {Mao}, M.~Y. and {McConnell}, D. and 
	{Norris}, R.~P. and {Schnitzeler}, D. and {Subrahmanyan}, R. and 
	{Urquhart}, J.~S. and {Thompson}, M.~A. and {Wark}, R.~M.},
    title = "{The Australia Telescope Compact Array Broad-band Backend: description and first results}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.3532},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: interferometers, methods: observational, ISM: general, galaxies: general, radio continuum: general, radio lines: general},
     year = 2011,
    month = sep,
   volume = 416,
    pages = {832-856},
      doi = {10.1111/j.1365-2966.2011.19054.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.416..832W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.382..382M,
   author = {{Murphy}, T. and {Mauch}, T. and {Green}, A. and {Hunstead}, R.~W. and 
	{Piestrzynska}, B. and {Kels}, A.~P. and {Sztajer}, P.},
    title = "{The second epoch Molonglo Galactic Plane Survey: compact source catalogue}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0708.3092},
 keywords = {methods: data analysis, catalogues, surveys, Galaxy: general, radio continuum: ISM},
     year = 2007,
    month = nov,
   volume = 382,
    pages = {382-392},
      doi = {10.1111/j.1365-2966.2007.12379.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382..382M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974A&AS...15..417H,
   author = {{H{\"o}gbom}, J.~A.},
    title = "{Aperture Synthesis with a Non-Regular Distribution of Interferometer Baselines}",
  journal = {\aaps},
     year = 1974,
    month = jun,
   volume = 15,
    pages = {417},
   adsurl = {http://adsabs.harvard.edu/abs/1974A%26AS...15..417H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980A&A....89..377C,
   author = {{Clark}, B.~G.},
    title = "{An efficient implementation of the algorithm 'CLEAN'}",
  journal = {\aap},
 keywords = {Algorithms, Data Processing, Image Processing, Radio Astronomy, Run Time (Computers), Astronomical Photography, Computer Techniques, Fast Fourier Transformations, Iterative Solution, Very Large Array (Vla)},
     year = 1980,
    month = sep,
   volume = 89,
    pages = {377},
   adsurl = {http://adsabs.harvard.edu/abs/1980A%26A....89..377C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1999ASPC..180..151C,
   author = {{Cornwell}, T. and {Braun}, R. and {Briggs}, D.~S.},
    title = "{Deconvolution}",
booktitle = {Synthesis Imaging in Radio Astronomy II},
     year = 1999,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 180,
   editor = {{Taylor}, G.~B. and {Carilli}, C.~L. and {Perley}, R.~A.},
    pages = {151},
   adsurl = {http://adsabs.harvard.edu/abs/1999ASPC..180..151C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

